Inverse problems and uncertainty quantification

In a Bayesian setting, inverse problems and uncertainty quantification (UQ) - the propagation of uncertainty through a computational (forward) model - are strongly connected. In the form of conditional expectation the Bayesian update becomes computationally attractive. This is especially the case as together with a functional or spectral approach for the forward UQ there is no need for time-consuming and slowly convergent Monte Carlo sampling. The developed sampling-free non-linear Bayesian update is derived from the variational problem associated with conditional expectation. This formulation in general calls for further discretisation to make the computation possible, and we choose a polynomial approximation. After giving details on the actual computation in the framework of functional or spectral approximations, we demonstrate the workings of the algorithm on a number of examples of increasing complexity. At last, we compare the linear and quadratic Bayesian update on the small but taxing example of the chaotic Lorenz 84 model, where we experiment with the influence of different observation or measurement operators on the update.

==> common/pdfsetup.tex <==
% RCSID:       $Id: pdfsetup.tex 36 2007-04-12 15:00:01Z opajonk $
% Author:      Oliver Pajonk
% Contact:     o.pajonk@tu-bs.de, oliver@oliverpajonk.de

% Setup PDF-Latex to fill in all relevant metadata into a PDF file
%
% Needs: - you have to declare \theauthor, \thetitle, \thesubject
%           \pdflinkcolor and  \thekeywords before including this file

% The following package defines \ifpdf properly even with MikTeX 2.5
\usepackage{ifpdf}

\ifpdf
  \usepackage[pdftex,
       colorlinks=true,		% use links with color instead of boxes
       bookmarksnumbered,	% bookmarks have numbers in front of topic
       bookmarksopen,		% opens the bookmarks when the PDF is opened
       pdfstartview=FitH,	% opens the PDF with 'fit width' view
       linkcolor=\pdflinkcolor,	% standard red
       citecolor=\pdflinkcolor,	% standard green
       urlcolor=\pdflinkcolor,	% standard cyan
       filecolor=\pdflinkcolor,	% ?
       hyperindex,		% ?
       plainpages=false,	% ?
       breaklinks=true,		% allow links to break across lines!
       pdfpagelabels, %?
       hypertexnames=true,
%        linktocpage=true  % if enabled the link in toc is placed on the number rather than on the text
     ]{hyperref}
     \pdfinfo{
        /Title (\thetitle)
        /Author (\theauthor)
        /Subject (\thesubject)
        /Keywords (\thekeywords)}
     \usepackage[dvipdf]{graphicx}
	 \usepackage[pdftex]{thumbpdf}
\else
  \usepackage[
    colorlinks=true,
    linkcolor=\pdflinkcolor,
    hyperindex,
    plainpages=false
  ]{hyperref}
  \usepackage[dvips]{graphicx}
\fi

\hypersetup{a5paper,
            colorlinks,
            linkcolor=\pdflinkcolor,
            citecolor=\pdflinkcolor,
            urlcolor=\pdflinkcolor,
            pdftitle={\thetitle},
            pdfauthor={\theauthor},
            pdfsubject={\thesubject},
            pdfkeywords={\thekeywords},
            pdfproducer={\theauthor~using \LaTeXe}}

